User Customizable and Robust Geo-Indistinguishability for Location Privacy

Location obfuscation functions generated by existing systems for ensuring location privacy are monolithic and do not allow users to customize their obfuscation range. This can lead to the user being mapped in undesirable locations (e.g., shady neighborhoods) to the location-requesting services. Modifying the obfuscation function generated by a centralized server on the user side can result in poor privacy as the original function is not robust against such updates. Users themselves might find it challenging to understand the parameters involved in obfuscation mechanisms (e.g., obfuscation range and granularity of location representation) and therefore struggle to set realistic trade-offs between privacy, utility, and customization. In this paper, we propose a new framework called, CORGI, i.e., CustOmizable Robust Geo-Indistinguishability, which generates location obfuscation functions that are robust against user customization while providing strong privacy guarantees based on the Geo-Indistinguishability paradigm. CORGI utilizes a tree representation of a given region to assist users in specifying their privacy and customization requirements. The server side of CORGI takes these requirements as inputs and generates an obfuscation function that satisfies Geo-Indistinguishability requirements and is robust against customization on the user side. The obfuscation function is returned to the user who can then choose to update the obfuscation function (e.g., obfuscation range, granularity of location representation). The experimental results on a real dataset demonstrate that CORGI can efficiently generate obfuscation matrices that are more robust to the customization by users.

==> customization.tex <==
\section{Customizing the matrix}


Upon receiving a robust obfuscation matrix (per Def. \ref{def:deltaPrune}), the system at the user end   prunes  away  entries in the matrix per the user policy  preferences.  Next, the matrix is updated according to  the precision level specified in the policy, in order to share the privatized location at the required  granularity.


\subsection{Matrix Precision Reduction}
\label{sect:precisionreduction}

\begin{figure}
    \centering
    \includegraphics[width=1.00 \linewidth]{fig/precisionreduction.pdf}
    \caption{Matrix precision reduction.}
    \label{fig:precisionreduction}
\end{figure}

Users can also choose the granularity at which their location should be shared using $Precision_l$ in the policy.
In Figure~\ref{fig:precisionreduction}, the original obfuscation matrix is generated for level 0 i.e., the set of leaf nodes. 
Suppose the user specifies $l$ as $Precision_l$, \emph{matrix precision reduction} generates the obfuscation matrix at level $l$, $\vMatrix{l}{}$ ($l > 0$), given the obfuscation matrix at level $0$, $\vMatrix{0}{}$.
As illustrated in the figure, the new matrix is generated by replacing all the rows of the descendant leaf nodes by their corresponding ancestor nodes at level $l$.
For each pair of nodes $\vNode{}{i}$ and $\vNode{}{j}$ at level $l$, we use $\children{\vNode{}{i}}$ and $\children{\vNode{}{j}}$ to represent the set of their descendant leaf nodes, respectively. 
The probability of selecting $\vNode{}{j}$ as the obfuscated location given the real location $\vNode{}{i}$ is calculated using Bayes' theorem.

\begin{eqnarray}{\label{eq:precisionReduction}}
\vCell{l}{i,j} 
&=& \frac{\sum_{\vNode{}{m} \in \children{\vNode{}{i}}} \vPrior{\vNode{}{m}} \sum_{\vNode{}{n} \in \children{\vNode{}{j}}} \vCell{0}{m, n}}{\vPrior{\vNode{}{i}}}
\end{eqnarray}

where $\vPrior{\vNode{}{m}}$ and $\vPrior{\vNode{}{i}}$ denote the prior distributions of $\vNode{}{m}$ and $\vNode{}{i}$ respectively. Note that, $\vPrior{\vNode{}{i}} = \sum_{\vNode{}{m} \in \children{\vNode{}{i}} } \vPrior{\vNode{}{m}}$.

\begin{proposition}
\label{prop:precisionreduction}
Matrix precision reduction preserves both probability unit measure and $\epsilon$-Geo-Ind. 
\end{proposition}
\begin{proof}
The proof can be found in Appendix. 
\end{proof}

\begin{algorithm}[t]
    \SetAlgoLined
    \DontPrintSemicolon
    \SetKwFunction{FMain}{precisionReduction}
    \SetKwProg{Fn}{Function}{:}{}  
    \small 
    \KwInput{Obfuscation matrix (at level 0) $\vMatrix{}{0}$, Location Tree $\vTree{}$, Prior Probability Distribution of Leaf Nodes $Prob^0$,  Precision Level $l$}
    \KwOutput{Obfuscation Matrix (at level k) $\vMatrix{}{k}$}
    \Fn{\FMain{$\vMatrix{}{0}$, $\vTree{}$, $Prob^0$, $l$}}{
        $\vNodeSet{l}$ = getNodes($\vTree{}$, $l$) \Comment{Get nodes at precision level} \\ 
        $\vMatrix{k}{}[0, 0] \ldots [\vCount{ \vNodeSet{l} } - 1, \vCount{\vNodeSet{l}} - 1]$ = 0 \\
        \For{$i$ $\in$ $0, \ldots, \vCount{\vNodeSet{l}} -1$}
        {   
            \For{$j$ $\in$ $0, \ldots, \vCount{\vNodeSet{l}} - 1$}
            {
                    $num = 0, den$ = 0 \\
                    \For{$u$ $\in$ $0 \ldots \mid \children{\vNode{}{i}} \mid - 1$}
                    {
                    $row\_sum$ = 0 \\
                    \For{$v$ $\in$ $0 \ldots \mid \children{\vNode{}{j}} \mid - 1$}
                    {
                    $row\_sum$ = $row\_sum + \vCell{0}{u, v}$
                    } 
            $num$ = $num + Prob^0[u] \times row\_sum$ \\
            $den = den + Prob^0[u]$  \\
            }
            $\vCell{k}{i, j}$ = $\frac{num}{den}$ \\
            }
        }
        \Return{$\vMatrix{k}{}$}
    }
    \caption{Precision Reduction Function}
    \label{alg:precisionReduction}
\end{algorithm}

Algorithm~\ref{alg:precisionReduction} presents the approach for matrix precision reduction given the matrix for leaf nodes ($\vMatrix{}{0}$), the location tree ($\vTree{}$), the prior probability distribution of the leaf nodes $prob^0$, and the precision level ($l$) which specifies the granularity/height of the tree of the reported location.
First, we get the set of nodes ($\vNodeSet{l}$) from level $l$ (Step 2).
We initialize the new obfuscation matrix with dimensions based on the set of nodes retrieved.
For each pair of location nodes ($\vNode{}{i}, \vNode{}{j}$) in $\vNodeSet{l}$, we compute their corresponding probability in the new matrix ($\vCell{k}{i,j}$) by using the probabilities of their leaf nodes, $\children{\vNode{}{i}}$ and $\children{\vNode{}{j}}$ respectively, in Equation~\ref{eq:precisionReduction} (Steps 4-16).
Finally, the new matrix $\vMatrix{l}{}$ for level $l$ is returned.
Thus using matrix precision reduction, we are able to save the overhead of generating the obfuscation matrix when user chooses to share at a lower granularity than the leaf nodes.


